One-Bit Coherent Distributed Radar Detection in Clutter via Velocity-Plane Search: Vanishing Loss and EEC-Calibrated Thresholding

Coherent distributed radar architectures enhance the detectability of low-reflectivity targets. However, conventional coherent processing generally entails prohibitively large volumes of inter-station data exchange, thereby motivating the adoption of one-bit quantization strategies. In this work, we investigate a clutter-dominated regime in which the interference is driven by a dense ensemble of weak scatterers. We demonstrate that, under these conditions, one-bit quantization can exhibit a vanishing performance loss with respect to ideal high-resolution sampling in terms of detection capability, in contrast to the classical 2 dB performance penalty associated with one-bit detection in white Gaussian noise environments. For unknown target velocity, we reformulate joint velocity-search processing under the effective one-bit model. Maximizing over the velocity plane makes false-alarm calibration an extreme-value problem for a correlated two-dimensional random field, whose maximum is not characterized by its pointwise null distribution alone. We therefore use an expected Euler characteristic approximation to calibrate the search threshold. We obtain analytic expressions for a separable two-station geometry and use constrained coefficient fitting for larger networks. Monte Carlo simulations demonstrate negligible quantization loss in the clutter-dominated setting and conservative false-alarm calibration under the tested Gaussian slow-time model.

==> def.tex <==
%\usepackage{amsfonts, amsmath, mathrsfs,  amssymb, dsfont, mathtools, slashbox, pifont, amsbsy, graphicx, url, algorithmic, yfonts, bbm, amssymb,amsmath}
%\usepackage[all,dvips,arc,curve,color,frame]{xy}
%\usepackage[dvips]{color}
%\usepackage[numbers]{natbib}
%\usepackage[numbers]{natbib}
%\usepackage[noadjust]{cite}
%\usepackage{pifont}
\usepackage{amsfonts, amsmath, mathrsfs, amsbsy, amssymb, dsfont, color}
\usepackage{graphicx}
%\usepackage{cite}
%\usepackage[all,dvips,arc,curve,color,frame]{xy}
%\usepackage{url}
%\usepackage{algorithm,algorithmic}

\newcommand\prefixtext[1]{%
  \ifvmode\else\\\@empty\fi
  \noalign{%
    \penalty0%
    \vbox{\mathstrut}%
    \penalty10000%
    \vskip-\baselineskip
    \penalty10000%
    \vbox to 0pt{%
      \normalbaselines
      \ifdim\linewidth=\columnwidth
      \else
        \parshape\@ne
        \@totalleftmargin\linewidth
      \fi
      \vss
      \noindent#1\par}%
      \penalty10000%
      \vskip-\baselineskip}%
      \penalty10000}

%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}

%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{definition}[1][Definition]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{example}[1][Example]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{remark}[1][Remark]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

\newcommand{\qed}{\nobreak \ifvmode \relax \else
      \ifdim\lastskip<1.5em \hskip-\lastskip
      \hskip1.5em plus0em minus0.5em \fi \nobreak
      \vrule height0.75em width0.5em depth0.25em\fi}

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\newcommand{\comment}[1]{}
% \newcommand{\davidsays}[1] {{\bf{\textcolor{blue}{DAVID SAYS: [#1]}}}}
\newcommand{\davidsays}[1]{}
\newcommand{\here} {{\bf{\textcolor{magenta}{Heeeeere }}}}
\newcommand{\YH}[1] {{\bf{\textcolor{mygreen}{[#1]}}}}
\def\({\left(}
\def\){\left)}
\def\bal{\pmb{\mathscr{\alpha}}}
\def\bbe{\boldsymbol{\beta}}
\def\bga{\boldsymbol{\gamma}}
\def\bde{\boldsymbol{\delta}}
\def\bep{\boldsymbol{\epsilon}}
\def\bvep{\boldsymbol{\varepsilon}}
\def\bze{\boldsymbol{\zeta}}
\def\bet{\boldsymbol{\eta}}
\def\bth{\boldsymbol{\theta}}
\def\bvth{\boldsymbol{\vartheta}}
\def\bio{\boldsymbol{\iota}}
\def\bka{\boldsymbol{\kappa}}
\def\bla{\boldsymbol{\lambda}}
\def\bmu{\boldsymbol{\mu}}
\def\bnu{\boldsymbol{\nu}}
\def\bo{\boldsymbol{o}}
\def\bpi{\boldsymbol{\pi}}
\def\bPi{\boldsymbol{\Pi}}
\def\bvpi{\boldsymbol{\varpi}}
\def\brh{\boldsymbol{\rho}}
\def\bvrh{\boldsymbol{\varrho}}
\def\bsi{\boldsymbol{\sigma}}
\def\bvsi{\boldsymbol{\varsigma}}
\def\bta{\boldsymbol{\tau}}
\def\bup{\boldsymbol{\upsilon}}
\def\bph{\boldsymbol{\phi}}
\def\bvph{\boldsymbol{\varphi}}
\def\bch{\boldsymbol{\chi}}
\def\bps{\boldsymbol{\psi}}
\def\bom{\boldsymbol{\omega}}
\def\bGa{\boldsymbol{\Gamma}}
\def\bDe{\boldsymbol{\Delta}}
\def\bTh{\boldsymbol{\Theta}}
\def\bth{\boldsymbol{\theta}}
\def\btau{\boldsymbol{\tau}}
%\def\bth{\mathbf{\theta}}
\def\bLa{\boldsymbol{\Lambda}}
\def\bXi{\boldsymbol{\Xi}}
\def\bxi{\boldsymbol{\xi}}
\def\bPh{\boldsymbol{\Phi}}
\def\bSi{\boldsymbol{\Sigma}}
\def\bUp{\boldsymbol{\Upsilon}}
\def\bPh{\boldsymbol{\Phi}}
\def\bPs{\boldsymbol{\Psi}}
\def\bOm{\boldsymbol{\Omega}}
\def\tr{\text{tr}}
\def\({\left(}
\def\){\right)}
\def\[{\left[}
\def\]{\right]}
\def\BEq{\begin{eqnarray}}
\def\EEq{\end{eqnarray}}
\def\BE*{\begin{eqnarray*}}
\def\EE*{\end{eqnarray*}}
\def\BA{\begin{array}}
\def\EA{\end{array}}
%\def\XN{\begin{align}}
%\def\YN{\end{align}}
\def\TAG{\addtocounter{equation}{1} \tag{\theequation}}
\def\Nn{\nonumber}
\def\0{\mathbf{0}}
\def\1{\mathbf{1}}
\def\a{\mathbf{a}}
\def\A{\mathbf{A}}
\def\sA{\pmb{\mathscr{A}}}
\def\bA{\mathbb{A}}
\def\b{\mathbf{b}}
\def\B{\mathbf{B}}
\def\sB{\pmb{\mathscr{B}}}
\def\bB{\mathbb{B}}
\def\c{\mathbf{c}}
\def\C{\mathbf{C}}
\def\sC{\pmb{\mathscr{C}}}
\def\bC{\mathbb{C}}
\def\d{\mathbf{d}}
\def\D{\mathbf{D}}
\def\sD{\pmb{\mathscr{D}}}
\def\sL{\pmb{\mathscr{L}}}
\def\bD{\mathbb{D}}
\def\e{\mathbf{e}}
\def\E{\mathbf{E}}
\def\sE{\pmb{\mathcal{E}}}
\def\sE{\pmb{\mathscr{E}}}
\def\bE{\mathbb{E}}
\def\f{\mathbf{f}}
\def\tf{\pmb{f}}
\def\F{\mathbf{F}}
\def\sF{\pmb{\mathscr{F}}}
\def\tF{\pmb{\mathcal{F}}}
\def\bF{\mathbb{F}}
\def\g{\mathbf{g}}
\def\G{\mathbf{G}}
\def\h{\mathbf{h}}
\def\H{\mathbf{H}}
%\def\i{\pmb{i}}
%\def\i{\mathbf{i}}
\def\I{\mathbf{I}}
\def\j{\mathbf{j}}
\def\J{\mathbf{J}}
\def\sJ{\pmb{J}}
\def\k{\mathbf{k}}
\def\K{\mathbf{K}}
\def\l{\mathbf{l}}
\def\L{\mathbf{L}}
\def\sL{\pmb{\mathscr{L}}}
\def\m{\mathbf{m}}
\def\M{\mathbf{M}}
\def\n{\mathbf{n}}
\def\N{\mathbf{N}}
%\def\o{\mathbf{o}}
\def\O{\mathbf{O}}
\def\p{\mathbf{p}}
\def\P{\mathbf{P}}
\def\q{\mathbf{q}}
\def\Q{\mathbf{Q}}
\def\r{\mathbf{r}}
\def\sr{\pmb{{r}}}
\def\R{\mathbf{R}}
\def\sR{\pmb{\mathscr{R}}}
\def\tR{\pmb{\mathcal{R}}}
\def\bR{\mathbb{R}}
\def\s{\mathbf{s}}
\def\S{\mathbf{S}}
\def\t{\mathbf{t}}
\def\T{\mathbf{T}}
\def\u{\mathbf{u}}
\def\U{\mathbf{U}}
\def\sU{\pmb{\mathscr{U}}}
\def\bU{\mathbb{U}}
\def\v{\mathbf{v}}
\def\V{\mathbf{V}}
\def\w{\mathbf{w}}
\def\W{\mathbf{W}}
\def\x{\mathbf{x}}
\def\X{\mathbf{X}}
\def\y{\mathbf{y}}
\def\Y{\mathbf{Y}}
\def\z{\mathbf{z}}
\def\Z{\mathbf{Z}}
\def\De{\mathbf \Delta}
\def\bZe{\mathbf \Zeta}
\def\sinc{{\rm sinc}}
\def\vec{{\rm vec}}
\def\mod{{\rm mod}}
\def\tx{\pmb{x}}
\def\sX{\pmb{\mathscr{X}}}
\def\tX{\pmb{\mathcal{X}}}
\def\sY{\pmb{\mathscr{Y}}}
\def\tY{\pmb{\mathcal{Y}}}
\def\sy{\pmb{y}}
\def\sz{\pmb{z}}
\def\ty{\pmb{\mathfrak{y}}}
%\def\tU{\tilde{\U}_s}
\def\dU{\bDe\U_s}
\def\tV{\tilde{\V}_s}
\def\dV{\bDe\V_s}
\def\tL{\tilde{\bLa}_s}
\def\dL{\Delta\bLa_s}
\def\Un{\tilde{\U}_n}
\def\Vn{\tilde{\V}_n}
\def\sD{\pmb{\mathcal{D}}}
\def\sB{\pmb{\mathcal{B}}}
\def\ha{\hat{\a}}
\def\hb{\hat{\b}}
\def\Wa{\W_{\a}}
\def\Wb{\W_{\b}}
\def\tP{\pmb{\mathcal{P}}}
\def\tA{\pmb{\mathcal{A}}}
\def\tWa{\pmb{\mathcal{W}}_a}
\def\tW{\pmb{\mathcal{W}}}
\def\tH{\pmb{\mathcal{H}}}
\def\uG{\pmb{\mathbb{G}}}
\def\uH{\pmb{\mathbb{H}}}
\def\sW{\pmb{\mathscr{W}}}
\def\sG{\pmb{\mathscr{G}}}
\def\sH{\pmb{\mathscr{H}}}
\def\hb{\pmb{\mathscr{\hbar}}}
\def\tG{\pmb{\mathcal{G}}}
\def\tg{\pmb{\mathcal{g}}}
\def\th{\pmb{\mathcal{h}}}
\def\sc{\pmb{c}}
\def\ss{\pmb{s}}
%\def\gb{\pmb{\textbarg}}
\def\fa{\pmb{\mathfrak{a}}}
\def\fb{\mathfrak{b}}
\def\tU{\pmb{\mathds{U}}}
\def\tV{\pmb{\mathcal{V}}}
\def\tS{\pmb{\mathcal{S}}}
\def\sU{\pmb{\mathscr{U}}}
\def\sV{\pmb{\mathscr{V}}}
\def\su{\pmb{u}}
\def\sv{\pmb{v}}
\def\ttU{\tilde{\pmb{\mathcal{U}}}}
\def\ttV{\tilde{\pmb{\mathcal{V}}}}
\def\DU{\bDe{\pmb{\mathcal{U}}}}
\def\tu{{\pmb{u}}}
\def\Du{\bDe{\pmb{u}}}
\def\tfa{\tilde{\mathfrak{a}}_1}
\def\hfa{\hat{\mathfrak{a}}_k}
\def\sA{\pmb{\mathscr{A}}}
\def\sB{\pmb{\mathscr{B}}}
\def\tfb{\tilde{\mathfrak{b}}_1}
\def\hfb{\hat{\mathfrak{b}}_k}
\def\hS{\hat{\S}}
\def\wh{{\rm where}}
\def\wh{\prefixtext{where}}
\def\and{\prefixtext{and}}
\def\Toep{{\rm Toeplitz}}
\def\su{\pmb{u}}
\def\sg{\pmb{g}_k\(\mu_k\)}
\def\sh{\pmb{h}_k\(\nu_k\)}
\def\bg{\mathfrak{g}}
\def\bh{\mathfrak{h}}
\def\hg{{\pmb{g}}}
\def\hh{{\pmb{h}}}
\def\sa{\pmb{a}}
\def\bP{\mathfrak{\Psi}}
\def\ta{\pmb{\textgoth{a}}}
\def\tb{{\textgoth{b}}}
\def\ts{\pmb{s}}
\def\tc{\pmb{\textfrak{c}}}
\def\gu{\pmb{\textswab{u}}}
\def\gv{\pmb{\textswab{v}}}
\def\gU{\pmb{\textswab{U}}}
\def\gV{\pmb{\textswab{V}}}
\def\hu{\pmb{\mathbbmtt{u}}}
\def\diag{{\rm diag}}
\def\Diag{{\rm Diag}}
\def\sZ{\pmb{\mathscr{Z}}}
\def\tZ{\pmb{\mathcal{Z}}}
\def\ha{{\mathscr{\mathbb{a}}}}
\def\tx{\pmb{x}}
\def\sz{\pmb{z}}
\def\etr{\textrm{etr}}
\def\Im{\mathrm{Im}}
\def\Re{\mathrm{Re}}

